Inverse Problems: A Deterministic Approach using Physics-Based Reduced Models

These lecture notes summarize various summer schools that I have given on the topic of solving inverse problems (state and parameter estimation) by combining optimally measurement observations and parametrized PDE models. After defining a notion of optimal performance in terms of the smallest reconstruction error that any reconstruction algorithm can achieve, the notes present practical numerical algorithms based on nonlinear reduced models for which one can prove that they can deliver a performance close to optimal. We also discuss algorithms for sensor placement with the approach. The proposed concepts may be viewed as exploring alternatives to Bayesian inversion in favor of more deterministic notions of accuracy quantification.

==> residual-based-surrogates.tex <==
%%%%%%%%%%%%%%%%%%%%
\newcommand{\rrZ}{r_{\mbox{\tiny Z}}}
%\newcommand{\rrV}{r_{\mbox{\tiny V}}}
%%%%%%%%%%%%%%%%%%%%%%
{The computational  realization of the above concepts hinges on two main constituents, namely (i)  the ability to evaluate bounds $\e_n$ for 
$\dist (\cM,V_n)$ as well as  (ii)  to have at hand computationally affordable surrogates ${\cal S}(v,\cM)$ for $\dist (v,\cM)= \min_{u\in \cM}\|v -u\|$.
In both cases one exploits the fact that errors in $V$ are equivalent to residuals in a suitable dual norm. Regarding (i), the derivation of bounds
$\e_n$ has been discussed extensively in the context of Reduced Basis Methods \cite{RHP}, see also \cite{DPW} for
the more general framework discussed below. Substantial   computational effort in an offline phase 
provides residual based surrogates for  $\|u-u(y)\|$  permitting frequent parameter queries at an online stage needed, in particular, to construct
reduced bases. This strategy becomes challenging though for high parameter dimensionality and we refer to \cite{CDDN} for remedies based
on trading deterministic certificates against probabilistic ones at significantly reduced computational cost. Therefore, we focus here on task (ii).
}
 


One typical setting where a computable surrogate $\cS(v,\cM)$ can be derived is when
$u(y)$ is the solution to a parametrized operator equation of the general form
\begin{equation}
A(y)u(y)=f(y).
\end{equation}
Here we assume that for every $y\in Y$ the right side $f(y)$ belongs
to the dual $Z'$ of a Hilbert test space $Z$, and $A(y)$ is boundedly invertible from $V$ to $Z'$.
The operator equation has therefore an equivalent variational formulation
\begin{equation}
\label{varform}
\cA_y(u(y),v)=\cF_y(v), \quad v\in Z,
\end{equation}
with parametrized bilinear form $\cA_y(w,v)=\<A(y)w,v\>_{Z',Z}$ and linear form $\cF_y(v)=\<f(y),v\>_{Z',Z}$.
This setting includes classical elliptic problems with $Z=V$,
as well as saddle-point and {unsymmetric problems such as convection-diffusion problems or space-time formulations of parabolic problems}.

We assume continuous dependence of $A(y)$ and $f(y)$ with respect to $y\in Y$, which by compactness of $Y$,
implies uniform boundedness and invertibility, that is
\begin{equation}
\|\cA(y)\|_{V\to Z'}\leq R\quad {\rm and}\quad \|\cA(y)^{-1}\|_{Z'\to V}\leq r^{-1}, \quad y\in Y,
\label{boundA}
\end{equation}
for some $0<r\leq R<\infty$. It follows that for any $v\in V$, one has the equivalence
\begin{equation}
\label{rR}
r\|v-u(y)\|_V \leq \cR(v,y) \leq R\|v-u(y)\|_V.
\end{equation}
where
\begin{equation}
\cR(v,y):=\|A(y)v-f(y)\|_{Z'},
\label{resid}
\end{equation} 
is the residual of the PDE for a state $v$ and parameter $y$.

Therefore the quantity
\begin{equation}
\label{surrS}
\cS(v,\cM):=\min_{y\in Y}\cR(v,y),
\end{equation}
provides {us} with a surrogate of $\dist(v,\cM)$ that satisfies the required framing \eqref{surframe}.

One first advantage of this surrogate quantity is that for each given $y\in Y$,
the evaluation of the residual $\|A(y)v-f(y)\|_{Z'}$ does not require to compute the solution $u(y)$.
Its second advantage is that the minimization in $y$ is facilitated in the relevant case where
$A(y)$ and $f(y)$ have affine dependence on $y$, that is,
\begin{equation}
A(y)=A_0 +\sum_{j=1}^d y_jA_j\quad {\rm and} \quad f(y)=f_0+\sum_{j=1}^d y_j f_j.
\label{affine}
\end{equation}
Indeed, $\cS(v, \cM)$ then amounts to the minimization over $y\in Y$ of the function 
\begin{equation}
\label{Rvy0}
\cR(v,y)^2:=\Big\|A_0v-f_0+\sum_{j=1}^d y_j(A_j v-f_j)\Big\|_{Z'}^2,
\end{equation}
which is a convex quadratic polynomial in $y$. {Hence, a minimizer $y(v)\in Y$ of the corresponding constrained linear least-squares problem exists, rendering the surrogate $\cS(v,\cM)= \cR(v,y(v))$ well-defined.}

{In all the above mentioned examples the norm $\|\cdot\|_Z = \langle\cdot,\cdot\rangle_Z^{1/2}$ can be efficiently computed.  For instance, in the simplest case of an $H^1_0(\Omega)$-elliptic problem 
one has $Z=V = H^1_0(\Omega)$ with 
\begin{equation}
\langle v,z\rangle_Z = \int_\Omega \nabla v\cdot\nabla z dx.
\end{equation} 
The obvious obstacle is then, however, the computation of the {\em dual norm} $\|\cdot\|_{Z'}$ which in the particular example  above is the $H^{-1}(\Omega)$-norm. A viable strategy is to use} {the Riesz lift $\rrZ: Z'\to Z$, defined by
\begin{equation}
\label{Riesz}
\langle \rrZ g,z\rangle_Z = \<g,z\>_{Z',Z}= g(z),\quad g\in Z',\, z\in Z,
\end{equation}
{which implies} that $\|\rrZ g\|_Z = \|g\|_{Z'}$. {Thus, $\cR(v, y)^2$
is computed for
a given $(v, y)\in V\times Y$ by introducing the lifted elements} 
\begin{equation}
\label{ej}
e_j \coloneqq \rrZ(A_jv- f_j),\quad j=0,\ldots,d,
\end{equation}
so that, by linearity
\begin{equation}
\label{Q}
\cR(v,y)^2 = \Big\| e_0 + \sum_{j=1}^d y_j e_j\Big\|^2_Z .
\end{equation}
}

{Note that} the above derivation is still idealized {as the $d+1$ variational problems \eqref{ej} are posed 
in the infinite dimensional space $Z$. As} already stressed in Remark \ref{spacediscretization}, all computations take place
in  {reference finite element spaces $V_h\subset V$ and $Z_h\subset Z$}. We thus approximate 
the $e_j$ by $e_{j,h}\in Z_h$, for $v\in V_h$,
using the Galerkin approximation of \eqref{Riesz}.
 This gives rise to a computable least-squares functional 
 \begin{equation} \label{Rvy0h}
\cR_h(v,y)^2 = \Big\| e_{0,h} + \sum_{j=1}^d y_j e_{j,h}\Big\|^2_Z ,\quad y\in Y.
\end{equation}
The practical distance surrogate is then defined through the
corresponding constrained least-squares problem 
\begin{equation} \label{Svy0h}
\cS_h(v,\cM_h):= \min_{y\in Y}\cR_h(v,y),
\end{equation}
which can be solved by
standard optimization methods. As indicated earlier,  the recovery schemes can be interpreted as taking place in a fixed discrete setting, with $\cM$ replaced by $\cM_h$,
comprised of approximate solutions in a large finite element space $V_h\subset V$, and measuring accuracy only in this
finite dimensional setting. 
One should note though that the approach allows one to disentangle
discretization errors from recovery estimates, even with regard to the underlying continuous PDE model.
In fact,  given any target tolerance $\e_h$, using a posteriori error control in $Z$, the spaces $V_h,Z_h$ can be chosen large enough
to guarantee that
\begin{equation}
\label{eh}
\big|\cR(v,y) - \cR_h(v,y) \big| \le \e_h\|v\|,\quad v\in V_h.
\end{equation}
Accordingly,   one  has $\big|\cS_h(v,\cM_h)- \cS(v,\cM)\big|\le \e_h\|v\|$, so that recovery estimates remain
meaningful with respect to the continuous setting as long as $\e_h$ remains sufficiently dominated
by the the threshholds $\e_k, \sigma, \e_{\rm noise}$ appearing in the above results. For notational simplicity
we therefore continue working in the continuous setting.

